Maximum Gain Round Trips with Cost Constraints

Searching for optimal ways in a network is an important task in multiple application areas such as social networks, co-citation graphs or road networks. In the majority of applications, each edge in a network is associated with a certain cost and an optimal way minimizes the cost while fulfilling a certain property, e.g connecting a start and a destination node. In this paper, we want to extend pure cost networks to so-called cost-gain networks. In this type of network, each edge is additionally associated with a certain gain. Thus, a way having a certain cost additionally provides a certain gain. In the following, we will discuss the problem of finding ways providing maximal gain while costing less than a certain budget. An application for this type of problem is the round trip problem of a traveler: Given a certain amount of time, which is the best round trip traversing the most scenic landscape or visiting the most important sights? In the following, we distinguish two cases of the problem. The first does not control any redundant edges and the second allows a more sophisticated handling of edges occurring more than once. To answer the maximum round trip queries on a given graph data set, we propose unidirectional and bidirectional search algorithms. Both types of algorithms are tested for the use case named above on real world spatial networks.

==> a.tex <==
A maximum gain round trip is different from other similar types of
network queries. A round trip in our definition is a way and thus,
it is allowed to pass by the nodes and edges more than once. Thus,
it is different from finding Euler or Hamilton paths in a graph.
An important issue about our problem definition is the possibility
to traverse the same edge for an arbitrary amount of times.
Depending on the given task, this might lead to round trips having
a large redundancy in the number of visited edges. Therefore, we
distinguish our problem further into two sub problems: The first
allows edges to be visited several times and thus simply maximizes
the gain while keeping the cost below the given threshold $\tau$.
In the second setting, the definition of round trips is extended
by allowing that each edge in the round trip is visited at most
$k$ times. Furthermore, each edge is considered only once when
calculating the gain without consideration of any additional
traversal.

\begin{figure*}[t]
\centering \fbox{
  \begin{minipage}{0.98\textwidth}
  \sf\scriptsize
   SimpleMGRQ(Node $s$, Float $tau$)\\
   (1)quad\hspace*{0em}Nodetab  tab  = InitNotetab()\\
   (2)quad\hspace*{0em}PriorityQueue queue = InitQueue()\\
   (3)quad\hspace*{0em}FOR EACH Link $l$ IN $s.outlinks()$ DO \\
   (4)quad\hspace*{1em}Way $w$ = new $Way(s,l)$
   (5)quad\hspace*{1em}$tab.update(w)$\\
   (6)quad\hspace*{1em}$queue.update(w.last,w.gain)$\\
   (7)quad\hspace*{0em}END FOR\\
   (8)quad\hspace*{0em}WHILE NOT $queue.isEmpty()$ DO\\
   (9)quad\hspace*{1em}Entry $entry =queue.pop()$\\
   (10)quad\hspace*{1em}List<Way> aktList = entry.getUndominated()\\
   (11)quad\hspace*{1em}aklist = removeProcessedWays(aktlist) \\
   (12)quad\hspace*{1em}setProcessed(aktlist)\\
   (13)quad\hspace*{1em}List<Way> candidates =
   extendWays(aktList)\\
   (14)quad\hspace*{1em}FOR EACH $w$ IN candidates DO \\
   (15)quad\hspace*{2em}IF $w.cost < \tau$ DO \\
   (16)quad\hspace*{3em}$tab.update(w)$\\
   (17)quad\hspace*{3em}$queue.update(w.last,w.gain)$\\
   (18)quad\hspace*{2em}END IF\\
   (19)quad\hspace*{1em}END FOR\\
   (20)quad\hspace*{0em}END WHILE\\
   (21)quad\hspace*{0em}RETURN $tab.getEntry(s)$\\
\end{minipage}
} \caption{Pseudocode of the simple MGRQ Algorithm}
\label{code:algorithm1}
\end{figure*}


==> algorithms_old.tex <==
\section{Algorithms}\label{sec:}
In section \ref{sec:rtbs} we first explain a naive breath first search approach with global pruning as a baseline for our evaluation.
In section \ref{sec:rtsc} we describe the skyline approach using local and global pruning. Our new algorithm using dual search of forth and back paths is then presented in section \ref{sec:rtfb}.
For all methods we assume that the user defines a certain accepted cost constraint $C_{max}$ in terms of distance or travel time along to the query, so that all round trips should be found that are closest to this cost constraint.

\subsection{RTBS: Round Trip Basic Search}\label{sec:rtbs}
The first algorithm is based on a breadth first search of the graph.
This method uses a priority queue $Q$, with the routes with lowest cost being on top of the queue.
$Q$ is initialized with the trivial path $p$ containing only the source node $n_1$.

Then, the first path is removed from $Q$ and expanded by all $n$ outgoing links of the last element of $p$, thus building $n$ new paths $p_i$.
If one of the new paths contains a link more than $k$-times, it is rejected immediately without further processing.
All remaining expanded paths are then checked, if their approximated cost
\begin{align*}
cost_{approx}(p) = cost(p) + \hat{D}(last(p),n_1)
\end{align*}
exceeds $C_{max}$ and if the last element of $p$ ($=last(p)$) equals to the source node $n_1$:
%
If
\begin{align}\label{eq:costApproximation}
0.9~C_{max} < cost_{approx}(p) <= C_{max} ~\wedge~ last(p) = n_1
\end{align}
holds, then $p$ is added to the result set $S_{Result}$.
%
Otherwise, if $cost_{approx}(p) > C_{max}$ and thus exceeds the accepted cost,
then $p$ is rejected.
%
Else if $cost_{approx}(p) < C_{max}$ and if $last(p) \neq n_1$, then $p$ is added to $Q$ as it has not yet reached the start node and still does not exceed the maximum allowed cost criteria.

This loop continues until $Q$ is empty.
If the cost criteria is given as a distance, the euclidean distance between the last element of $p$ to the start node can be used as in Definition \ref{def:networkDistanceEstimation}. If the cost criteria is
defined by a temporal constraint, the euclidean distance between the first and last element of the path needs to be divided by the maximum possible speed of the traveler and thus leads to an analogous approximation to $n_1$.

When all candidate paths in $Q$ have been processed, $S_{Result}$ contains all
round trips that have been identified. $S_{Result}$ can then be ordered by the
benefit of each path and returned to the user.





\subsection{RTSC: Round Trip Skyline Computation}\label{sec:rtsc}
As RTBS does not make use of any local pruning, the amount of candidates in
the queue grows very fast. Thus we need to make use of global and local
pruning which is the case when the search is done by using skyline computation and according forward estimations.


\subsubsection{Forward Approximation}
While RTBS used an forward approximation for the minimum cost of $p$ when it is extended in the shortest/fastest possible way back to the start node, there is also the possibility to make an approximation for the benefit of $p$:
As we aim at maximizing the benefit of $p$, an approximation for an an upper
bound is needed, so that all paths can be pruned, that cannot outperform $p$
even if they achieve the maximum reachable benefit.

The approximated benefit $benefit_{approx}(p)$ of a path $p$ can be obtained
by adding the already determined $benefit(p)$ to the maximal expected benefit
of $p$. As can be seen in Equation \eqref{eq:benefit}, the benefit is defined by the preference vector and the according edge.
In order to define an upper bound of the benefit, we thus need to approximate the maximum benefit, that a path $p$ can reach until it hits the start node.
As the cost and thus the length of the desired round trip is limited, we can approximate $benefit_{approx}(p)$ by multiplying the maximal preference vector by the maximal remaining cost:
\begin{align}
benefit_{approx}(p) &= benefit(p) + \Pi^T \cdot \theta_{max}(\hat{e}) \label{eq:maxBenefit}\\
\hat{e}          &= (last(p), n_1)
\end{align}
with $\hat{e}$ being a virtual edge which realizes the path from the currently last node of $p$ back to the start node by acquiring the maximally allowed
cost: $ cost(\hat{e}) = C_{max} - cost(p)$.
$\theta_{max}$ is the maximum preference vector, where each component
$\theta_i$ is set to the maximum value.

Finally, this approximation can be used in order to achieve a global pruning, as soon as a complete round trip has been identified.
If all already found round trips are stored in a skyline $S_{Result}$, it is checked, whether or not the currently approximated path $p$ is dominated by any $p_s \in S_{Result}$.
If $p$ is dominated by any $p_s$, then $p$ does not need to be processed any more will be pruned. Otherwise, $p$ remains in the candidate set and will be processed.


\subsubsection{Sub Skyline Pruning}
One drawback of the forward approximation is that it can only be applied if there is already at least one path in the result set.
Thus we use another pruning criterion that can be applied even if the result set is empty:

Given two paths $p = (n_1, \ldots, n_i)$, $q = (n_1, \ldots, n_i)$ so that $p \neq q$ (which is for example the case if $n_i$ is reachable by two different paths), it can be checked whether or not $p$ and $q$ have a dominance relationship according to their current cost and benefit.
According to \cite{SchRenKri10}, pruning can already be applied even if $n_i \neq n_1$, so that the round trip does not need to be finished.
If $p$ and $q$ have a dominance relationship, then only one path needs to be processed in the further computation, while the dominated path can be pruned from further computation as it can never yield a better result than its' dominating path. Thus, $p$ can be pruned from further processing, if
$cost(p) > cost(q)$ and $benefit(p) < benefit (q)$ (cf. Figure \ref{fig:pruningarea}).
\begin{figure}
    \centering
        \includegraphics[width=0.20\textwidth]{figures/pruningarea}
    \caption{Visualization of the skyline and the pruning area of a point $d$ on the skyline. The pruning area is visualized by the grey rectangle and the dashed lines.}
    \label{fig:pruningarea}
\end{figure}


\subsubsection{Round Trip Search}\label{sec:rtscSearch}
hier dann nochmal der pseudoalgorithmus mit lokalem pruning und vorwärtsabschätzung


\subsection{RTFB: Round Trip Forth and Back}\label{sec:rtfb}
Both RTBS and RTSC use a minimum approximation for the path cost that can be expected as defined in Equation \eqref{eq:costApproximation}.
The drawback of this minimum approximation is, that the pruning power is of course smaller than the real distance, so that the search space grows larger
than needed in all cases where $cost_{approx}(p) < cost(p)$ holds for a completed round trip path $p$.

In order to overcome this drawback, we modify RTSC by splitting the computation into two phases: In the first phase, forth and back routes are computed separately, which are then connected to complete round trips in the second phase.
The intention is, that even though we cannot apply global pruning in phase 1 as no complete round trips are produced until phase 2, the search space is reduced as we do not a minimum approximation but only the real cost.

\subsubsection{Computation of forth and back paths}
In this first phase, forth and back routes are computed simultaneously with
the cost constraint set to $C_h = \frac{C_{max}}{2}$ but in difference to
RTSC, the computation is done without any forward approximation.
In order to obtain paths that are as close as possible to the cost criteria, a
forth path $p$ is expanded as long as it does not exceed the cost criteria
$C_h$. At the time, where $p= (n_1, \ldots, n_i)$ is expanded to $p'= (n_1,
\ldots, n_i, n_j)$ and exceeds $C_h$ for the first time (which means that
$cost(p) \leq C_h < cost(p')$), $p'$ is added to the set of forth paths $S_F$.
All paths $p \in S_F$ are not expanded any further in this phase.

The computation of the back routes is done analogous to the forth routes with
the difference, that the expansion stops one step earlier. This means that a
back route $p$ is expanded as long as $cost(p) < C_h$. As soon as an expansion
of $p$ to $p'$ leads to $p < C_h \leq q'$, the expansion of $p$ is stopped and
$p$ is added to the result set of back routes $S_B$. As $e = (n_i, n_j) \neq
(n_j, n_i) = \hat{e}$, it needs to be ensured that the back routes are
directed in that way, that they end in $n_1$ ($last(p) = n_1$) as this also
affects the computation of $cost(p)$.


SONDERFALL: es darf nichts gepruned werden das min. einen link doppelt enthält. Grund: sonderfall von matthias, dass auch ein rückweg eine der doppelkanten AUCH NOCH besuchen will. BILD NÖTIG!

\begin{figure}[htbp]
  \centering
  \subfigure[]{
    \label{fig:rtfb_a}
<<<<<<< .mine
    \includegraphics[width=0.14\textwidth]{figures/rtfb_pruning}
=======
    \includegraphics[width=0.14\textwidth]{figures/rtfb_pruning1} 
>>>>>>> .r39
  }
  \subfigure[]{
    \label{fig:rtfb_b}
    \includegraphics[width=0.14\textwidth]{figures/rtfb_pruning1_a}
  }
  \subfigure[]{
    \label{fig:rtfb_c}
    \includegraphics[width=0.14\textwidth]{figures/rtfb_pruning1_b}
  }
  \caption{RTFB local pruning problem }
  \label{fig:rtfb_local_pruning}
\end{figure}
\subsubsection{Concatenation}

